Batch Value-function Approximation with Only Realizability

We make progress in a long-standing problem of batch reinforcement learning (RL): learning $Q^\star$ from an exploratory and polynomial-sized dataset, using a realizable and otherwise arbitrary function class. In fact, all existing algorithms demand function-approximation assumptions stronger than realizability, and the mounting negative evidence has led to a conjecture that sample-efficient learning is impossible in this setting (Chen and Jiang, 2019). Our algorithm, BVFT, breaks the hardness conjecture (albeit under a stronger notion of exploratory data) via a tournament procedure that reduces the learning problem to pairwise comparison, and solves the latter with the help of a state-action partition constructed from the compared functions. We also discuss how BVFT can be applied to model selection among other extensions and open problems.

==> figures/ms_table.tex <==
%!TEX root = ../paper.tex

\begin{table}[t]
\begin{tabular}{|p{2cm}|p{2.5cm}|c|c|c|c|}
\hline
\textbf{Method} & \textbf{Base Alg.}  & \textbf{Surrogate for $J(\pi)$}  & \tabincell{c}{Additional Assumptions} & \textbf{Stat.~Error} &  \textbf{Allowed $|F|$} \\ \hline
Abstraction Selection & Model-based w/ abstractions  & \begin{tabular}[c]{@{}c@{}}Bisimulation error\\ of base algorithms\end{tabular} & None                                                                       & Poly                 & Constant             \\ \hline
		\begin{tabular}[c]{@{}c@{}}BFVT\\ (this work)\end{tabular}      & \begin{tabular}[c]{@{}c@{}}Algorithms that\\ approximate Q\end{tabular} & f - Q                                                                           & None                                                                       & Poly                 & Exp.                 \\ \hline
		OPE-IS                                                          & \multirow{2}{*}{Any}                                                    & \multirow{2}{*}{J()}                                                            & None                                                                       & Exp. in horizon      & Exp.                 \\ \cline{1-1} \cline{4-6} 
		OPE-MIS                                                         &                                                                         &                                                                                 & \begin{tabular}[c]{@{}c@{}}Q in \\ (or stronger)\end{tabular}              & Poly                 & Exp.                 \\ \hline
	\end{tabular}
\end{table}
